Contextual bandits with concave rewards, and an application to fair ranking

We consider Contextual Bandits with Concave Rewards (CBCR), a multi-objective bandit problem where the desired trade-off between the rewards is defined by a known concave objective function, and the reward vector depends on an observed stochastic context. We present the first algorithm with provably vanishing regret for CBCR without restrictions on the policy space, whereas prior works were restricted to finite policy spaces or tabular representations. Our solution is based on a geometric interpretation of CBCR algorithms as optimization algorithms over the convex set of expected rewards spanned by all stochastic policies. Building on Frank-Wolfe analyses in constrained convex optimization, we derive a novel reduction from the CBCR regret to the regret of a scalar-reward bandit problem. We illustrate how to apply the reduction off-the-shelf to obtain algorithms for CBCR with both linear and general reward functions, in the case of non-combinatorial actions. Motivated by fairness in recommendation, we describe a special case of CBCR with rankings and fairness-aware objectives, leading to the first algorithm with regret guarantees for contextual combinatorial bandits with fairness of exposure.

==> generic_aliases.tex <==
\RequirePackage{bbm}
\RequirePackage{mathtools}
\RequirePackage{stmaryrd}
\RequirePackage{xspace}
\RequirePackage{setspace}
\RequirePackage{amsfonts,amsmath,amssymb}
%%%%%%%%%%%%%%%%%%%%
% settings for enumitem
\RequirePackage{enumitem}
\setlist[itemize]{leftmargin=*,noitemsep,topsep=-\parskip+3pt}
\setlist[enumerate]{leftmargin=*,noitemsep,topsep=-\parskip+3pt}
%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%
% settings for subassumptions
\newtheorem{manualassumptioninner}{Assumption}
\newenvironment{manualassumption}[1]{%
  \renewcommand\themanualassumptioninner{#1}%
  \manualassumptioninner
}{\endmanualassumptioninner}

%%%%%%%%%%%%%%%%%%%%
% settings for algorithms
\usepackage[ruled,noline,linesnumbered]{algorithm2e}
\newcommand\mycommfont[1]{\rmfamily{#1}}
\SetCommentSty{mycommfont}
\setlength{\algomargin}{1em}
\SetInd{0em}{0.5em}
\RequirePackage{etoolbox}

\makeatletter
% Remove right hand margin in algorithm
\patchcmd{\@algocf@start}% <cmd>
  {-1.5em}% <search>
  {0pt}% <replace>
  {}{}% <success><failure>
\makeatother

%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%
%%%% thm
% \RequirePackage{amsthm}
% alternative to amsthm: thmtools
\RequirePackage{thmtools,thm-restate}
\makeatletter
\DeclareRobustCommand{\qed}{%
  \ifmmode % if math mode, assume display: omit penalty etc.
  \else \leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
  \fi
  \quad\hbox{\qedsymbol}}
\newcommand{\openbox}{\leavevmode
  \hbox to.77778em{%
  \hfil\vrule
  \vbox to.675em{\hrule width.6em\vfil\hrule}%
  \vrule\hfil}}
\newcommand{\qedsymbol}{\openbox}
\newenvironment{proof}[1][\proofname]{\par
  \normalfont
  \topsep6\p@\@plus6\p@ \trivlist
  \item[\hskip\labelsep\itshape
    #1.]\ignorespaces
}{%
  \qed\endtrivlist
}
\newcommand{\proofname}{Proof}
\makeatother
%%% end of thmtools
%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\indic}[1]{\mathbbm{1}_{\{#1\}}}
\renewcommand{\Re}{\mathbb{R}}
\newcommand{\Nat}{\mathbb{N}}
\newcommand{\expect}{\mathbb{E}}
\newcommand{\prob}{\mathbb{P}}




\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

\DeclarePairedDelimiter\intint{\llbracket}{\rrbracket}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}
\DeclarePairedDelimiter\card{|}{|}
\DeclarePairedDelimiter\xset{\{}{\}}


%dot product
\DeclarePairedDelimiterX\dotp[2]{\langle}{\rangle}{#1\,\delimsize\vert\,\mathopen{}#2}

% multiliner within an equation
\newcommand{\multiliner}[2]{\parbox{#1}{\setstretch{1}\centering#2}}

==> sections/old_vd_intro.tex <==
\section{Introduction}


While machine learning methods have been mostly developed with the goal of maximizing a single scalar reward, there is increasing pressure to insist on the multi-objective nature of many machine learning applications \citep{vamplew2018human,helberger2018exposure,barocas2017fairness,abdollahpouri2019beyond,rolf2020balancing,stray2021you}. From online recommendation platforms that optimize for several metrics of user satisfaction \citep{mehrotra2020bandit,ribeiro2012pareto,agarwal2011click,lakiotaki2011multicriteria} to fairness concerns in recommender systems \citep{mehrotra2018towards,burke2018balanced,ekstrand2022fairness,abdollahpouri2019unfairness}, the ability to learn while maintaining optimal trade-offs between several objectives is a key component of modern machine learning systems. In this paper, we focus on the problem of online learning with bandit feedback and multiple rewards, where the desired trade-off between the rewards is defined by a known concave objective function, referred to as \emph{\textsc{b}andits with \textsc{c}oncave \textsc{r}ewards} (\bcr) \citep{agrawal2014bandits}. This setting is particularly relevant to fair machine learning in online allocation problems or recommender systems, where the overall welfare is naturally expressed as a (known) concave function of the (unknown) utilities of the agents \citep{moulin2003fair,berthet2017fast,do2021two}. 

% \alessandro{I would restructure as: introduce the problem / explain the main challenge (i.e., working on policy space) / mention the FW-based methods are promising but literature is unsatisfactory / explain the core technical approach / list the contributions}


% Our algorithm views \cbcr as an optimization problem in reward space, more precisely as a Frank-Wolfe (\FW) algorithm that maximizes the objective function over the convex set $\S$ of feasible expected rewards, i.e., the set of expected reward of all policies. Whereas \FW was already used for learning with concave rewards since \citet{agrawal2014bandits} \citep[also see][]{berthet2017fast,cheung2019regret}, the novelty of our analysis is an explicit characterization of the support function of $\S$, i.e., the mapping $\g\mapsto\maxs \g^\intercal\s$, which relates the \FW update direction to the expected rewards of actions taken at a given time step.

In this paper, we focus on stochastic \emph{\textsc{c}ontextual} \bcr{} (\cbcr), where the reward vector depends on an observed stochastic context. This extension of \bcr is required in real-world problems such as recommendation systems, where the context contains the user/item features that are required to personalize the recommendations.
The main challenge of \cbcr is that the optimal stationary policy depends on the entire distribution of contexts and reward. In contrast, in scalar-reward contextual bandits, an optimal policy is to greedily maximize the reward at each context. In \bcr, since there are no contexts, existing approaches directly optimize over distribution of actions \citep{agrawal2014bandits,berthet2017fast}. These are not applicable to \cbcr because it would require explicit representations of stationary policies as mappings from contexts to distribution of actions. To our knowledge, the only prior theoretical work on \cbcr is restricted to finding the best policy within a finite set \citep{agrawal2016efficient}.

We present \emph{the first algorithms with provably vanishing regret} for \cbcr without restriction on the policy space. Our main theoretical result is a reduction where the \cbcr regret of an algorithm is bounded by its regret on a proxy bandit task with \emph{single} (scalar) reward -- more precisely a contextual bandit with adversarial contexts and stochastic rewards, a problem that has been extensively studied. This reduction shows that it is straightforward to turn \emph{any} contextual (scalar reward) bandits into algorithms for \cbcr. \virginie{is it useful to say how the reduction works here in the intro, or is this unnecessary abstract?} We prove this reduction by first re-parameterizing \cbcr as an optimization problem in the space of feasible rewards, and then revealing connections between Frank-Wolfe (\FW) optimization in reward space and a decision problem in action space. This removes the need for explicit representations of policies altogether. 

We provide two examples for \cbcr with non-combinatorial actions, for linear bandits based on LinUCB \citep{abbasi2011improved}, but also for general reward functions based on the work of \citet{foster2020beyond} using online regression oracles. In particular, we highlight that our reduction can be used together with any exploration/exploitation principle, while previous \FW approaches to bandits or reinforcement learning with concave rewards relied exclusively on upper confidence bounds \citep{agrawal2014bandits,berthet2017fast,cheung2019regret}.

One of our main motivations for addressing \cbcr is the question of fairness of exposure, which has received a lot of attention recently \citep{biega2018equity,morik2020controlling,singh2018fairness}, including from the bandit literature \citep{wang2021fairness,patil2020achieving,xu2021combinatorial}. We show how our reduction approach also applies to the combinatorial task of fair ranking in the contextual bandit setting. Fairness of exposure often consists in making trade-offs between average ranking performance and a measure of fairness for items \citep{do2021two}. Most of previous works focus on fairness constraints, while we allow for concave trade-off functions, which offer more flexibility. More importantly, these works are restricted to either multi-armed bandits without extension to ranking \citep{celis2018algorithmic,wang2021fairness,patil2020achieving,chen2020fair}, or apply to combinatorial bandits without context \citep{xu2021combinatorial}. Both these restrictions are impractical for recommender systems. \citep{mansoury2021unbiased,jeunen2021top} propose heuristics that apply to both ranking and contexts in this space, but they lack theoretical guarantees. Our work presents the \emph{first algorithm with regret guarantees for fair ranking with contextual bandits.}


% To showcase the versatility of our approach, we describe how it applies to a combinatorial linear bandit problem of fair ranking \citep{jeunen2021top,mansoury2021unbiased}. We study a framework where the goal is to make a trade-off between average ranking performance and a function promoting equal exposure of items \citep{do2021two}. The question of fairness of exposure has received a lot of attention recently \citep{biega2018equity,morik2020controlling,singh2018fairness}, including from the bandit literature \citep{wang2021fairness,patil2020achieving,xu2021combinatorial}. Most of these works focus on fairness constraints, while we allow for arbitrary concave functions, which offers more flexibility. More importantly, these works are restricted to either multi-armed bandits without extension to ranking \citep{celis2018algorithmic,wang2021fairness,patil2020achieving,chen2020fair}, or apply to combinatorial bandits without context \citep{xu2021combinatorial}. We present the first algorithm with regret guarantees that applies to both ranking and contexts in that space.



We provide a detailed discussion of the related work in Appendix~\ref{sec:related_work}. \virginie{Comment: From the reviews, I feel like we need a small related work paragraph in the main paper. Or maybe we should discuss related work more in the intro (I tried to add a bit)...
% I would use this related work section to:
% \begin{enumerate}
%     \item previous FW approaches in related BCR problems (since/ if we choose not to talk about FW anymore)
%     \item how our work generalizes theoretical works on CBCR or fair ranking bandits, or provides theoretical guarantees for empirical work
% \end{enumerate}
}

\virginie{Do we want FW in the title? How about: Contextual Bandits with Concave Rewards, and an application to fair ranking}


